Bidirectional Reactive Programming for Machine Learning

Reactive languages are dedicated to the programming of systems which interact continuously and concurrently with their environment. Values take the form of unbounded streams modeling the (discrete) passing of time or the sequence of concurrent interactions. While conventional reactivity models recurrences forward in time, we introduce a symmetric reactive construct enabling backward recurrences. Constraints on the latter allow to make the implementation practical. Machine Learning (ML) systems provide numerous motivations for all of this: we demonstrate that reverse-mode automatic differentiation, backpropagation, batch normalization, bidirectional recurrent neural networks, training and reinforcement learning algorithms, are all naturally captured as bidirectional reactive programs.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
all:  paper.pdf

paper.pdf:  paper.tex body.tex definitions.tex semantics_definitions.tex paper.bib sema-simul.tex supplementary.tex
	export TEXINPUTS=::/Users/dpotop/github/mlir-rt/papers/ReactiveML/graphics
	pdflatex paper
	bibtex paper
	pdflatex paper
	pdflatex paper
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex paper; done

clean:
	rm -f paper.pdf paper.bbl paper.blg  paper.log paper.out  paper.aux


